Recent Progress in Solar Atmospheric Neutrino Searches with IceCube

Cosmic-rays interacting with nucleons in the solar atmosphere produce a cascade of particles that give rise to a flux of high-energy neutrinos and gamma-rays. Fermi has observed this gamma-ray flux; however, the associated neutrino flux has escaped observation. In this contribution, we put forward two strategies to detect these neutrinos, which, if seen, would push forward our understanding of the solar atmosphere and provide a new testing ground of neutrino properties. First, we will extend the previous analysis, which used high-energy through-going muon events collected in the years of maximum solar activity and yielded only flux upper limits, to include data taken during the solar minimum from 2018 to 2020. Extending the analysis to the solar minimum is important as the gamma-ray data collected during past solar cycles indicates a possible enhancement in the high-energy neutrino flux. Second, we will incorporate sub-TeV events and include contributions from all neutrino flavors. These will improve our analysis sensitivity since the solar atmospheric spectrum is soft and, due to oscillation, contains significant contributions of all neutrino flavors. As we will present in this contribution, these complementary strategies yield a significant improvement in sensitivity, making substantial progress towards observing this flux.

==> preamble.tex <==
\abstract{
    Cosmic-rays interacting with nucleons in the solar atmosphere produce a cascade of particles that give rise to a flux of high-energy neutrinos and gamma-rays. Fermi has observed this gamma-ray flux; however, the associated neutrino flux has escaped observation. In this contribution, we put forward two strategies to detect these neutrinos, which, if seen, would push forward our understanding of the solar atmosphere and provide a new testing ground of neutrino properties. First, we will extend the previous analysis, which used high-energy through-going muon events collected in the years of maximum solar activity and yielded only flux upper limits, to include data taken during the solar minima from 2018 to 2020. Extending the analysis to the solar minima is important as the gamma-ray data collected during past solar cycles indicates a possible enhancement in the high-energy neutrino flux. Second, we will incorporate sub-TeV events and include contributions from all neutrino flavors. These will improve our analysis sensitivity since the solar atmospheric spectrum is soft and, due to oscillation, contains significant contributions of all neutrino flavors. As we will present in this contribution, these complementary strategies yield a significant improvement in sensitivity, making substantial progress towards observing this flux.
}
\FullConference{37$^{\rm{th}}$ International Cosmic Ray Conference (ICRC 2021)\\
		July 12th -- 23rd, 2021\\
		Online -- Berlin, Germany}
\author*[a]{Josh Villarreal}
\author[b]{Gerrit Roellinghoff}
\author[a,c]{Jeffrey Lazar}

\affiliation[a]{Department of Physics and Laboratory for Particle Physics and Cosmology, Harvard University\\Cambridge, MA 02138, USA}
\affiliation[b]{Dept. of Physics, Sungkyunkwan University\\Suwon 16419, Korea}
\affiliation[c]{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin–Madison\\Madison, WI 53706, USA}

\title{Recent Progress in Solar Atmospheric Neutrino Searches with IceCube}
\ShortTitle{Solar Atmoshperic Neutrinos with IceCube} 
\date{\today}


==> sections/results.tex <==
\subsection{Previous analysis}
A previous search for solar atmospheric neutrinos was done with 7 years of IceCube data (2010-2016) taken during the austral winter, when the declination of the Sun is above $-5^{\circ}$. Using a baseline flux from \cite{Edsjo2017}, they set a 90\% upper limit of $1.02^{+0.20}_{-0.18}\cdot10^{-13}$~$\mathrm{GeV^{-1}cm^{-2}s^{-1}}$ at 1~\textrm{TeV}. Out of 7 years, only 6 were using the full 86 string detector configuration, and the analysis time period was only during times of increased solar activity. They observed an under-fluctuation of the data at $1.8 \sigma$ significance, with the resulting upper limit set at an order of magnitude larger than their chosen baseline flux. \cite{Jin2021}
\subsection{Sensitivity for new analysis}
We evaluate our sensitivities at the 90\% confidence level using the Neyman method \cite{Neyman1937}. Table \ref{table:sens} shows our integrated flux sensitivities for our reference fluxes from \cite{FJAW2017,Edsjo2017}. Depending on the flux model, the resulting sensitivities are 2-4 times the model flux, with the main difference between \cite{FJAW2017,Edsjo2017} being the lower total integrated flux for \cite{FJAW2017}.

\begin{table}[h]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|c|c|}
\hline
                           & Sens. in units of model flux & Sens. at 1 TeV [GeV$^{-1}$ cm$^{-2}$ s$^{-1}$] \\ \hline
Edsjo2017 \cite{Edsjo2017} & 2.61                         & $1.72 \cdot 10^{-14}$                          \\
FJAW2017  \cite{FJAW2017}  & 3.51                         & $1.95 \cdot 10^{-14}$                          \\ \hline
\end{tabular}%
}
\caption{Sensitivities to reference solar atmospheric flux models from \cite{FJAW2017,Edsjo2017}. Sensitivities are given in units of model flux and for the corresponding value at 1 TeV.}
\label{table:sens}
\end{table}

We also calculate the differential sensitivity in half-decade energy bins, assuming our reference flux from \cite{FJAW2017} for 9 years (2011-2020). We omit calculating the differential flux for \cite{Edsjo2017}, since shape similarity between both theoretical models means the sensitivities are nearly identical. To look at the sensitivity to a possible change in flux hardness during periods of low solar activity, we also calculate the differential sensitivity for a power-law flux with $\Gamma=2.2$ for 2017-2020 as a naive extrapolation of the Fermi-LAT solar minimum data. The differential sensitivities are shown in Figure \ref{pic:diff} alongside gamma-ray flux and limits from HAWC \cite{Albert2018} and Fermi-LAT \cite{Linden_2018}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/diff.pdf}
    \caption{Differential sensitivity in half-decade energy bins for reference flux from FJAW2017 \cite{FJAW2017} for 9 years of data and for 3 years of low solar activity (2017-2020) using a power law with $\Gamma =2.2$ as a naive extrapolation of Fermi-LAT solar minimum data \cite{Linden_2018}. Also shown are gamma-ray results from HAWC \cite{Albert2018} and Fermi-LAT \cite{Linden_2018}.}
    \label{pic:diff}
\end{figure}

==> sections/selections.tex <==
\todo{Is it necessary to have a new chapter for the small text about the event selection? -H}
For high energy events, we use a new IceCube dataset using 9 years of 86-string data from 2011 to 2020, notably including the solar minimum of 2018-2020. This IceCube dataset features an improved energy reconstruction and angular reconstruction compared to previous samples, and all 9 years feature the full detector configuration CITE[INT]. The event selection is limited to upgoing events (sun declination $\delta_{sun} > -5^{\circ}$), using the Earth as an effective atmospheric muon veto to create a high-purity neutrino sample. It uses only $\nu_{\mu} + \bar{\nu}_{\mu}$ track events, owing to their superior angular reconstruction at high-energies. 
% Figure \ref{pic:two_plot} shows the expected event rate depending on energy E$_{\nu}$ and reconstructed distance from the sun $\Psi$.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\textwidth]{figures/two_plot.pdf}
%     \caption{Expected distribution in neutrino energy E$_{\nu}$ and reconstructed distance from the sun $\Psi$ for up-going high-energy neutrino based on MC data.}
%     \label{pic:two_plot}
% \end{figure}
